Revizor: Testing Black-box CPUs against Speculation Contracts

Speculative vulnerabilities such as Spectre and Meltdown expose speculative execution state that can be exploited to leak information across security domains via side-channels. Such vulnerabilities often stay undetected for a long time as we lack the tools for systematic testing of CPUs to find them. In this paper, we propose an approach to automatically detect microarchitectural information leakage in commercial black-box CPUs. We build on speculation contracts, which we employ to specify the permitted side effects of program execution on the CPU's microarchitectural state. We propose a Model-based Relational Testing (MRT) technique to empirically assess the CPU compliance with these specifications. We implement MRT in a testing framework called Revizor, and showcase its effectiveness on real Intel x86 CPUs. Revizor automatically detects violations of a rich set of contracts, or indicates their absence. A highlight of our findings is that Revizor managed to automatically surface Spectre, MDS, and LVI, as well as several previously unknown variants.

==> 9a_demo_files.tex <==
% -*- root: ms.tex -*-

\section{Complete Contract Specifications}
\label{app:contracts}

This appendix details all contracts used in the paper.
The concrete instructions included in each class depend on the target instructions set.

\subsection{\memseq{}}\label{app:memseq}

\begin{lstlisting}[label={lst:memseq},style=embedded,language=yaml]
observation_clause: MEM
  - instructions: MemReads
    format: READ (ADDR), DEST
    observation: expose(ADDR)
  - instructions: MemWrites
    format: WRITE SRC, (ADDR)
    observation: expose(ADDR)
execution_clause: SEQ
  None
\end{lstlisting}

\subsection{\memcond{}}\label{app:memcond}

\begin{lstlisting}[label={lst:memcond},style=embedded,language=yaml]
observation_clause: MEM
  - instructions: MemReads
    format: READ (ADDR), DEST
    observation: expose(ADDR)
  - instructions: MemWrites
    format: WRITE SRC, (ADDR)
    observation: expose(ADDR)
execution_clause: COND
  - instructions: CondBranches
    format: COND_BR CONDITION (DEST)
    execution: {  # branch misprediction
      if NOT CONDITION then
          IP := IP + DEST
      fi
    }
\end{lstlisting}

\subsection{\ctseq{}}\label{app:ctseq}

\begin{lstlisting}[label={lst:ctseq},style=embedded,language=yaml]
observation_clause: CT
  - instructions: MemReads
    format: READ (ADDR), DEST
    observation: expose(ADDR)
  - instructions: MemWrites
    format: WRITE SRC, (ADDR)
    observation: expose(ADDR)
  - instructions: CondBranches
    format: COND_BR CONDITION (DEST)
    observation: {   # expose branch targets
      if CONDITION then
          expose(DEST)
      else
          expose(IP)
      fi
    }
execution_clause: SEQ
  None
\end{lstlisting}

\subsection{\ctcb{}}\label{app:ctcb}

\begin{lstlisting}[label={lst:ctcond},style=embedded,language=yaml]
observation_clause: CT
  - instructions: MemReads
    format: READ (ADDR), DEST
    observation: expose(ADDR)
  - instructions: MemWrites
    format: WRITE SRC, (ADDR)
    observation: expose(ADDR)
  - instructions: CondBranches
    format: COND_BR CONDITION (DEST)
    observation: {
      if CONDITION then
          expose(DEST)
      else
          expose(IP)
      fi
    }
execution_clause: COND
  - instructions: CondBranches
    format: COND_BR CONDITION (DEST)
    execution: {
      if NOT CONDITION then
          IP := IP + DEST
      fi
    }
\end{lstlisting}

\subsection{\ctcb{}-NonspeculativeStore}\label{app:ctcbstore}

\begin{lstlisting}[label={lst:ctcondstore},style=embedded,language=yaml]
observation_clause: CT-NonspeculativeStore
  - instructions: MemReads
    format: READ (ADDR), DEST
    observation: expose(ADDR)
  - instructions: MemWrites
    format: WRITE SRC, (ADDR)
    observation: {  # do not expose speculative stores
      if NOT IN_SPECULATION then
        expose(ADDR)
      fi
    }
  - instructions: CondBranches
    format: COND_BR CONDITION (DEST)
    observation: {
      if CONDITION then
          expose(DEST)
      else
          expose(IP)
      fi
    }
execution_clause: COND
  - instructions: CondBranches
    format: COND_BR CONDITION (DEST)
    execution: {
      if NOT CONDITION then
          IP := IP + DEST
      fi
    }
\end{lstlisting}

\newpage

\subsection{\ctsbp{}}\label{app:ctsbp}

\begin{lstlisting}[label={lst:ctbpas},style=embedded,language=yaml]
observation_clause: CT
  - instructions: MemReads
    format: READ (ADDR), DEST
    observation: ADDR
  - instructions: MemWrites
    format: WRITE SRC, (ADDR)
    observation: ADDR
  - instructions: CondBranches
    format: COND_BR CONDITION (DEST)
    observation: {
      if CONDITION then
          expose(DEST)
      else
          expose(IP)
      fi
    }
execution_clause: BPAS
  - instructions: MemWrites
    format: WRITE SRC, (ADDR)
    execution:
      # speculatively skip stores
      IP := IP + instruction_size()
\end{lstlisting}

\subsection{\ctcbsbp{}}\label{app:ctcbsbp}

\begin{lstlisting}[label={lst:ctcbsbp},style=embedded,language=yaml]
observation_clause: CT
  - instructions: MemReads
    format: READ (ADDR), DEST
    observation: expose(ADDR)
  - instructions: MemWrites
    format: WRITE SRC, (ADDR)
    observation: expose(ADDR)
  - instructions: CondBranches
    format: COND_BR CONDITION (DEST)
    observation: {
      if CONDITION then
          expose(DEST)
      else
          expose(IP)
      fi
    }
execution_clause: COND-BPAS
  - instructions: CondBranches
    format: COND_BR CONDITION (DEST)
    execution: {
      if NOT CONDITION then
          IP := IP + DEST
      fi
    }
  - instructions: MemWrites
    format: WRITE SRC, (ADDR)
    execution:
      # speculatively skip stores
      IP := IP + instruction_size()
\end{lstlisting}

\subsection{\ctrseq{}}\label{app:ctrseq}

\begin{lstlisting}[label={lst:ctrseq},style=embedded,language=yaml]
observation_clause:
  - instructions: RegReads  # expose register values
    format: READ SRC, DEST
    observation: expose(SRC)
  - instructions: MemReads
    format: READ (ADDR), DEST
    observation: expose(ADDR)
  - instructions: MemWrites
    format: WRITE SRC, (ADDR)
    observation: expose(ADDR)
  - instructions: CondBranches
    format: COND_BR CONDITION (DEST)
    observation: {
      if CONDITION then
          expose(DEST)
      else
          expose(IP)
      fi
    }
execution_clause:
  None
\end{lstlisting}

\subsection{\archseq{}}\label{app:archseq}

\begin{lstlisting}[label={lst:archseq},style=embedded,language=yaml]
observation_clause:
  - instructions: RegReads
    format: READ SRC, DEST
    observation: expose(SRC)
  - instructions: MemReads
    format: READ (ADDR), DEST
    observation: {
      expose(ADDR)
      expose(read(ADDR))  # expose loaded values
    }
  - instructions: MemWrites
    format: WRITE SRC, (ADDR)
    observation: expose(ADDR)
  - instructions: CondBranches
    format: COND_BR CONDITION (DEST)
    observation: {
      if CONDITION then
          expose(DEST)
      else
          expose(IP)
      fi
    }
execution_clause:
  None
\end{lstlisting}


\section{Example: Configuration File}
\label{app:example-config}

\begin{lstlisting}[label={lst:config-yaml},style=embedded,language=yaml]
# Generator
test_case_size: 8
max_mem_accesses: 4
min_bb_per_function: 3
max_bb_per_function: 3
supported_categories:
  - NOP
  - BINARY
  - BITBYTE
  - COND_BR
  - CMOV
  - CONVERT
  - DATAXFER
  - FLAGOP
  - SETCC
  - LOGICAL
  - POP
  - PUSH

# Model
contract_observation_mode: ct
contract_execution_mode:
  - seq

# Executor
attack_variant: P+P
enable_ssbp_patch: true
\end{lstlisting}

%\section{Example: Instruction Set Specification}
%\label{app:example-isa}
%
%
%\begin{figure*}[t]
%\begin{lstlisting}[label={lst:example-isa},style=embedded,language=XML]
%<root >
%  <extension ex="BASE">
%    <instruction asm="ADC" category="BINARY" cpl="3" extension="BASE">
%      <op idx="1" memory-prefix="byte ptr" r="1" type="mem" w="1" width="8" xtype="u8"/>
%      <op idx="2" r="1" type="imm" width="8"/>
%    </instruction>
%    <instruction asm="ADC" category="BINARY" cpl="3" extension="BASE" rex="0">
%      <op idx="1" r="1" type="reg" w="1" width="8">AL,CL,DL,BL,AH,CH,DH,BH</op>
%      <op idx="2" r="1" type="imm" width="8"/>
%    </instruction>
%    <instruction asm="REX ADC" category="BINARY" cpl="3" extension="BASE" rex="1">
%      <op idx="1" r="1" type="reg" w="1" width="8">GPR</op>
%      <op idx="2" r="1" type="imm" width="8"/>
%    </instruction>
%    ...
%    <instruction asm="CLI" category="FLAGOP" cpl="3" extension="BASE">
%    </instruction>
%    <instruction asm="CLTS" category="SYSTEM" cpl="0" extension="BASE">
%    </instruction>
%    <instruction asm="CMC" category="FLAGOP" cpl="3" extension="BASE">
%    </instruction>
%    ...
%\end{lstlisting}
%\end{figure*}

%\subsection{Example: Generated Test Case}
%\label{app:example-test-case}
%
%\input{listings/test-case.tex}


\section{Examples of Contract Violations}
\label{app:example-vulns}

This appendix shows examples of contract counterexamples generated by \sys{}.
\appref{example-v1} is the original generated test case, and the rest are automatically minimized versions.

\subsection{Instance of Spectre V1}
\label{app:example-v1}

\begin{lstlisting}[style=asm]
LEA R14, [R14 + 12] # instrumentation
MFENCE # instrumentation
.test_case_main.entry:
JMP .bb0
.bb0:
CMOVNL ECX, ECX
AND RBX, 0b0111111000000 # instrumentation
ADD RBX, R14 # instrumentation
ADC dword ptr [RBX], -67100032
NOT RAX
JP .bb1 # < ---------------------- mispredicted branch
JMP .test_case_main.exit
.bb1:
AND RBX, 1048197274
ADD AX, 5229
AND RCX, 0b0111111000000 # instrumentation
ADD RCX, R14 # instrumentation
ADC EAX, dword ptr [RCX] # < ----- speculative leak
{load} ADD RCX, RCX
.test_case_main.exit:
LEA R14, [R14 - 12] # instrumentation
MFENCE # instrumentation
\end{lstlisting}


\subsection{Minimized Instance of Spectre V4}
\label{app:example-v4}


\begin{lstlisting}[style=asm]
LEA R14, [R14 + 8] # instrumentation
MFENCE # instrumentation
.test_case_main.entry:
JMP .bb0
.bb0:
MOV RDX, 0 # leftover instrumentation
OR BX, 0x1c # leftover instrumentation
AND RAX, 0xff # leftover instrumentation
CMOVNZ BX, BX
AND RBX, 0b0111111000000 # leftover instrumentation
ADD RBX, R14 # leftover instrumentation
XOR AX, AX
AND RBX, 0b0111111000000 # instrumentation
ADD RBX, R14 # instrumentation
SETNS byte ptr [RBX]  # < ---------- delayed store
AND RAX, 0b0111111000000 # instrumentation
ADD RAX, R14 # instrumentation
MOVZX EDX, byte ptr [RAX]  # < ----- store bypass
AND RDX, 0b0111111000000 # instrumentation
ADD RDX, R14 # instrumentation
AND RCX, qword ptr [RDX]   # < ----- speculative leakage
LEA R14, [R14 - 8] # instrumentation
MFENCE # instrumentation
\end{lstlisting}

\subsection{Minimized Instance of MDS}
\label{app:example-mds}

\begin{lstlisting}[style=asm]
LEA R14, [R14 + 48] # instrumentation
MFENCE # instrumentation
.test_case_main.entry:
JMP .bb0
.bb0:
ADC EAX, -2030331421
AND RAX, 0b1111111000000 # instrumentation
ADD RAX, R14 # instrumentation
MOV CX, word ptr [RAX]  # < ---------- microcode assist
AND RCX, 0b1111111000000 # instrumentation
ADD RCX, R14 # instrumentation
SUB EAX, dword ptr [RCX]   # < ------- speculative leak
LEA R14, [R14 - 48] # instrumentation
MFENCE # instrumentation
\end{lstlisting}

\subsection{Minimized Instance of LVI-NULL}
\label{app:example-lvi}

\begin{lstlisting}[style=asm]
LEA R14, [R14 + 8] # instrumentation
MFENCE # instrumentation
.test_case_main.entry:
JMP .bb0
.bb0:
SUB AX, 27095
AND RAX, 0b1111111000000 # instrumentation
ADD RAX, R14 # instrumentation
ADD BL, byte ptr [RAX]  # < -- speculative zero injection
AND RBX, 0b1111111000000 # instrumentation
ADD RBX, R14 # instrumentation
OR dword ptr [RBX], -1193072838 # < ---- speculative leak
LEA R14, [R14 - 8] # instrumentation
MFENCE # instrumentation
\end{lstlisting}


\subsection{Minimized Instance of Spectre~V1-Var}
\label{app:example-v1-var}

\begin{lstlisting}[style=asm]
LEA R14, [R14 + 28] # instrumentation
MFENCE
.test_case_main.entry:
JMP .bb0
.bb0:
NOP
NOP
CDQ
SETZ CL
ADD EDX, 117
REX ADD BL, BL
SETNLE AL
SUB RBX, RBX
TEST AL, 29
MOV RDX, 0 # instrumentation
OR RBX, 0x6d # instrumentation
AND RAX, 0xff # instrumentation
DIV RBX  # < ---------------- variable-latency operation
{disp32} JNO .bb1
.bb1:
AND RCX, 0b111111000000 # instrumentation
ADD RCX, R14 # instrumentation
MOVZX EDX, byte ptr [RCX]
AND RAX, RAX
AND RAX, 0b111111000000 # instrumentation
ADD RAX, R14 # instrumentation
SBB qword ptr [RAX], 39412116
TEST ECX, ECX
AND RAX, 0b111111000000 # instrumentation
ADD RAX, R14 # instrumentation
MOV qword ptr [RAX], 81640764
REX NEG AL
CMC
OR RDX, 37323177
JNP .bb2  # < ---------------------- mispredicted branch
JMP .test_case_main.exit
.bb2:
REX SBB AL, AL
SBB EAX, 74935583
AND RDX, 0b111111000000 # instrumentation
ADD RDX, R14 # instrumentation
CMOVS RDX, qword ptr [RDX]     # < ---- speculative leak
AND RAX, 0b111111000000 # instrumentation
ADD RAX, R14 # instrumentation
MOV qword ptr [RAX], 23088010
AND RBX, 0b111111000000 # instrumentation
ADD RBX, R14 # instrumentation
LOCK AND word ptr [RBX], 5518 # < ---- speculative leak
.test_case_main.exit:
LEA R14, [R14 - 28] # instrumentation
MFENCE # instrumentation
\end{lstlisting}


\subsection{Minimized Instance of Speculative Store Eviction}
\label{app:example-v1-sstore}

\begin{lstlisting}[style=asm]
LEA R14, [R14 + 32] # instrumentation
MFENCE # instrumentation
.test_case_main.entry:
JMP .bb0
.bb0:
AND RBX, 0b0111111000000 # instrumentation
ADD RBX, R14 # instrumentation
LOCK AND dword ptr [RBX], EAX
JZ .bb1 # < ---------------------- mispredicted branch
JMP .test_case_main.exit
.bb1:
AND RAX, 0b0111111000000 # instrumentation
ADD RAX, R14 # instrumentation
MOV qword ptr [RAX], 3935 # < ---- speculative leak
.test_case_main.exit:
LEA R14, [R14 - 32] # instrumentation
MFENCE # instrumentation
\end{lstlisting}

\subsection{Minimized \ctrseq{} Violation}
\label{app:example-v1-ctr}

\begin{lstlisting}[style=asm]
LEA R14, [R14 + 4] # instrumentation
MFENCE # instrumentation
.test_case_main.entry:
JMP .bb0
.bb0:
{store} ADC CX, CX
AND RAX, 0b0111111000000 # instrumentation
ADD RAX, R14 # instrumentation
CMOVNS EBX, dword ptr [RAX]
AND RCX, 0b0111111000000 # instrumentation
ADD RCX, R14 # instrumentation
MOVZX ECX, byte ptr [RCX] # < --- non-speculative load
SUB RBX, 20
{store} ADC EDX, EDX
REX SETNLE AL
{store} REX ADC BL, BL
{disp32} JBE .bb1  # < ---------- branch misprediction
JMP .test_case_main.exit
.bb1:
REX INC AL
AND RCX, 0b0111111000000 # instrumentation
ADD RCX, R14 # instrumentation
MOV EBX, dword ptr [RCX]  # < ---- speculative leak
.test_case_main.exit:
LEA R14, [R14 - 4] # instrumentation
MFENCE # instrumentation
\end{lstlisting}


\subsection{Minimized \archseq{} Violation}
\label{app:example-v1-arch}

\begin{lstlisting}[style=asm]
LEA R14, [R14 + 60] # instrumentation
MFENCE # instrumentation
.test_case_main.entry:
JMP .bb0
.bb0:
{load} REX MOV DL, DL
MOVSX RBX, BX
{store} AND BX, BX
ADD EAX, 11839320
AND RDX, 0b0111111000000 # instrumentation
ADD RDX, R14 # instrumentation
SETS byte ptr [RDX]
TEST AX, 6450
AND RDX, 0b0111111000000 # instrumentation
ADD RDX, R14 # instrumentation
SUB word ptr [RDX], CX
{disp32} JB .bb1   # < ---------- branch misprediction
JMP .test_case_main.exit
.bb1:
SUB AX, -29883
AND RAX, 0b0111111000000 # instrumentation
ADD RAX, R14 # instrumentation
ADD EAX, dword ptr [RAX] # < ------- speculative load
AND RAX, 0b0111111000000 # instrumentation
ADD RAX, R14 # instrumentation
CMOVLE RBX, qword ptr [RAX] # < ---- speculative leak
.test_case_main.exit:
LEA R14, [R14 - 60] # instrumentation
MFENCE # instrumentation
\end{lstlisting}


==> tables/compare-cpus.tex <==
% -*- root: ../ms.tex -*-

\begin{table}[tp]
    \small
    \renewcommand{\arraystretch}{1.1}
    \center
    \begin{tabular}{c|c|cc}
        CPU & Skylake & \multicolumn{2}{c}{Coffee Lake} \\
        V4 patch & off & off & on \\
        \hline
        \hline
        \ctseq{} &     &     &    \\
        \ctsbp{} &     &     &    \\
        \hline
    \end{tabular}

    \caption{Testing hardware and firmware defences.
    The table shows the total number of violations detected on 10k test cases.}
    \label{tab:compare-cpus}
\end{table}

==> tables/fp.tex <==
% -*- root: ../ms.tex -*-

\begin{table}[tbp]
    \center
    \begin{tabular}{ll|cccc}
        Instr.  & Contract & Retires & Shuffles & False  & Unknown \\
        Set     &          &         &          & Posit. &         \\
        \hline
        \hline
        \ibc{}  & \ctseq   & 8       & 0        & 0      & 0       \\
        \ibm{}  & \ctsbp   & 10      & 0        & 0      & 0       \\
        \ibm{}  & \ctcbsbp & 5       & 0        & 0      & 0       \\
        \ibcm{} & \ctcbsbp & 65      & 45       & 2      & 21      \\
    \end{tabular}
    \caption{False positives. Numbers are per 1000 test cases.}
    \label{tab:fp}
\end{table}

==> tables/fuzzing-targets.tex <==
% -*- root: ../ms.tex -*-

\begin{table*}[tbp]
    \center
    \setlength{\tabcolsep}{3pt}
    \begin{tabular}{l||c|c|c|c|c|c||c|c}
        & Target 1 & Target 2 & Target 3 & Target 4 & Target 5 & Target 6 & Target 7 & Target 8 \\
        \hline
        \hline
        CPU & \multicolumn{6}{c||}{Skylake} & Skylake & \multicolumn{1}{c}{Coffee Lake} \\
        \hline
        V4 patch & \multicolumn{3}{c|}{off} & \multicolumn{3}{c||}{on} & \multicolumn{2}{c}{on} \\
        \hline
        Instruction Set & \ibasic & \ibm & \ibmv & \ibmv & \ibcm & \ibcmv & \multicolumn{2}{c}{\ibm} \\
        \hline
        Attack Mode & \multicolumn{6}{c||}{P+P} & \multicolumn{2}{c}{P+P+Assist} \\
        \hline
    \end{tabular}
    \caption{Description of the experimental setups.}
    \label{tab:targets}
\end{table*}


==> tables/observation-models.tex <==
% -*- root: ../ms.tex -*-

\begin{table}[tbp]
    \center
    \begin{tabular}{c|ccc}
        -       & L1D   & L1I     & ??? \\
        \hline
        \cseq   & \ibc  & \ibasic & ??? \\
        \csbp   & \ibm  & \ibm    & ??? \\
        \ccb    & \ibc  & \ibc    & ??? \\
        \ccbsbp & \ibcm & \ibcm   & ??? \\
    \end{tabular}
    \caption{The experiment illustrates how the contract bundle changes for different threat models.
    Each table entry is the instruction set which satisfies a given contract (row) under a given threat model (column).
    In this experiment, Speculative Store Bypass patch was disabled.}
    \label{tab:observation-models}
\end{table}


==> tables/speed.tex <==
% -*- root: ../ms.tex -*-

\begin{table}[tbp]
    \small
    \renewcommand{\arraystretch}{1.05}
%    \setlength{\tabcolsep}{3pt}
    \center
    \begin{tabular}{l|c|c|c|c}
        & Test          & Inputs & Eff. Classes & Pattern  \\
        Contract  & Cases         & / TC   & / TC         & Coverage \\
        \hline
        \hline
        \ctseq    & 5125          & 493    & 45           & 113,707k \\
        \ctsbp    & 5095          & 480    & 43           & 107,671k \\
        \ctcbsbp  & 5249          & 477    & 42           & 89,165k  \\
        \hline
    \end{tabular}
    \caption{Runtime parameters of a 24-hour testing campaign.
    \emph{Inputs/TC} is the average number of inputs per test case.
    \emph{Eff.Classes/TC} is the average number of effective input classes per test case. %, and in parentheses is the portion of effective classes among all classes.
    \emph{Pattern Coverage} is the number of covered pattern combinations.
    }
    \label{tab:speed}
\end{table}

